Failure Prediction with Statistical Guarantees for Vision-Based Robot Control

We are motivated by the problem of performing failure prediction for safety-critical robotic systems with high-dimensional sensor observations (e.g., vision). Given access to a black-box control policy (e.g., in the form of a neural network) and a dataset of training environments, we present an approach for synthesizing a failure predictor with guaranteed bounds on false-positive and false-negative errors. In order to achieve this, we utilize techniques from Probably Approximately Correct (PAC)-Bayes generalization theory. In addition, we present novel class-conditional bounds that allow us to trade-off the relative rates of false-positive vs. false-negative errors. We propose algorithms that train failure predictors (that take as input the history of sensor observations) by minimizing our theoretical error bounds. We demonstrate the resulting approach using extensive simulation and hardware experiments for vision-based navigation with a drone and grasping objects with a robotic manipulator equipped with a wrist-mounted RGB-D camera. These experiments illustrate the ability of our approach to (1) provide strong bounds on failure prediction error rates (that closely match empirical error rates), and (2) improve safety by predicting failures.

==> Fall21/conditional_probability.tex <==
\section{PAC-Bayes Bound with Conditional Probabilities}

Following from Section \ref{guaranteed}, we want to address the optimization problem of 
\begin{equation} \label{OPT}
\min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}} C_\pi (f; E) 
\end{equation}
However, we would like to generalize to the case of minimizing the conditional probabilities $\{p_{0 \rvert 1}, p_{1 \rvert 0} \}$, i.e. measure the gain of the detector. Currently, the cost function is 
\begin{equation}
    \begin{split}
        \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}} & \Big[p_{0 \cap 1} + p_{1 \cap 0} \Big] \\
        = & p_{0 \rvert 1}p_1 + p_{1 \rvert 0}p_0 \\
        = & (\lambda^*) p_{0 \rvert 1} + (1-\lambda^*)p_{1 \rvert 0}
    \end{split}
\end{equation}
In short, then, we would like to generalize these results to arbitrary $\lambda \in [0, 1]$. Ideally, we would like to maintain the standard PAC-Bayes type guarantees; however, the conditional probabilities must be estimated from $n_0$ and $n_1$ (number of successes and failures, respectively), where $N = n_0 + n_1$. In order to estimate this in an unbiased way, we need to scale the costs by $N/n_0$ and $N/n_1$. However, this causes problems in the standard PAC-Bayes analysis for two reasons: first, because the costs are no longer in $[0, 1]$, and second, because $n_0$ and $n_1$ are themselves random variables, and can only be estimated from the whole sample. \\

\noindent As such, we will devise an overestimate cost that holds with high probability and moves the randomness in $n_0$ and $n_1$ to the $1-\delta$ component of the bound. This transformation will also formalize the intuition that some minimum number each of failures and successes are necessary to make meaningful bounds on the conditional probabilities. In the primary formulation, this intuition is obviated by the observation that the joint probabilities are deflated by the empirical success (resp. failure) rate; as such, meaningful statements can be made about the joint probabilities even with no successes (resp. failures), as the low incident probability means that even a bad detector can only be wrong so many times. 

\subsection{Initial Setup and Bounding the Success/Failure}
Draw a sample $S_E$ of $N$ environments i.i.d. from some unknown $\mathbb{P}_\mathcal{E}$;  $S_E = \{E_i\}_{i=1}^N \overset{\text{i.i.d.}}{\sim} \mathbb{P}_\mathcal{E}^N$. Implicitly, each of these environments when combined (potentially) with fixed policy $\pi$ will induce a feature vector $x_i$ corresponding to the sensor measurements observed by the detector following $\pi$ in $E_i$. Let $x_i \in \mathcal{X}$. The fixed policy $\pi$ will also induce a success/failure label on each environment. \\

\noindent Let $\hat{p}_0, \hat{p}_1$ denote the empirical success/failure rates of $\pi$ on $S_E$. Fix $\lambda \in [0, 1]$ that denotes the relative importance of false positives and false negatives. From the sample size $N$, fixed $\lambda$, and chosen confidence level $\delta$, we can construct underestimates of the probabilities as $\underline{p}_0, \underline{p}_1$. We can use concentration inequalities to give a multiplicative bound whp on the empirical success/failure rates. From here, assume wlog $n_1 \leq n_0$.

\begin{lemma}
With probability $\geq 1-\delta$ over samples of size $N$, for any true $p_1$ and empirical lower bound $\underline{p}_1$, if the following definition for $K$ 
\begin{equation}
    1 < K \leq \underline{K} \triangleq \frac{3}{5} \bigg[\sqrt{\frac{N \underline{p}_1}{2\log{\frac{2}{\delta}}}}\bigg] = \bigg[\frac{3}{5\sqrt{2\log{\frac{2}{\delta}}}}\bigg] \sqrt{\underline{n}_1}
\end{equation}
is valid, then we have that $\hat{p}_1 \geq p_1\frac{K-1}{K}$ and $p_1 \geq \frac{K}{K+1} \hat{p}_1 = \hat{p}_1 - \frac{1}{K+1} \hat{p}_1$
\end{lemma}
\begin{proof}
The result follows from an application of Bernstein's inequality to the empirical mean of iid Bernoulli random variables. 

\noindent From the inequality: 
\begin{equation*}
\begin{split}
    \mathbb{P}\Big[\sum_{i=1}^N X_i - N\mu \geq t \Big] & \leq \text{exp}(\frac{-t^2}{2 \sum \sigma_i^2 + 2t/3}) = \delta \\
    \implies \log{\frac{1}{\delta}} & = \frac{t^2}{2N\sigma^2 + 2t/3} \\
    & \geq \min\{\frac{t^2}{4N\sigma^2}, \frac{3t}{4}\}
    \end{split}
\end{equation*}
This allows us to reason about $t$ as follows: 
\begin{equation*}
    \begin{split}
        \log{\frac{1}{\delta}} & \geq \frac{t^2}{4Np_1(1-p_1)} \\
        \implies t & \leq \sqrt{4Np_1(1-p_1)\log{\frac{1}{\delta}}}\text{, and} \\
        \log{\frac{1}{\delta}} & \geq \frac{3t}{4} \\
        \implies t & \leq \frac{4 \log{\frac{1}{\delta}}}{3}
    \end{split}
\end{equation*}
Therefore, w.p. $\geq 1-\delta$, we have that 
\begin{equation*}
    \mathbb{P}\Big[\sum_{i=1}^N X_i - N\mu \geq t \Big] \leq \delta 
\end{equation*}
where 
\begin{equation*}
    t = 2\sqrt{N\sigma^2\log{\frac{1}{\delta}}} + \frac{4\log{\frac{1}{\delta}}}{3}
\end{equation*}
And for $N \geq \frac{2 \log{\frac{1}{\delta}}}{p_1} \geq  \frac{\log{1/\delta}}{\sigma^2}$, we have that
\begin{equation*}
    \sqrt{N\sigma^2 \log{\frac{1}{\delta}}} \geq \log{\frac{1}{\delta}}
\end{equation*}
which implies that for $N \geq \frac{2 \log{\frac{1}{\delta}}}{p_1} \geq \frac{\log{1/\delta}}{\sigma^2}$, 
\begin{equation*}
    t \leq \frac{10}{3}\sqrt{N \sigma^2 \log{\frac{1}{\delta}}}
\end{equation*}
Switching to the empirical mean (i.e. dividing by $N$) and incorporating the `double-sided' Bernstein inequality (i.e. using an absolute value in the probability statement and substituting $2/\delta$ into the logarithm to account for an extra union bound), we have that 
\begin{equation*}
    \mathbb{P}\Big[\frac{1}{N}\sum_{i=1}^N X_i - \mu \geq \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{1}{\delta}}}{N}} \Big] \leq \delta 
\end{equation*}
and equivalently, that 
\begin{equation*}
\begin{split}
    \mathbb{P}\Big[\lvert \frac{1}{N}\sum_{i=1}^N X_i - \mu \rvert \geq \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{2}{\delta}}}{N}} \Big] & \leq \delta \\
    \mathbb{P}\Big[\lvert \hat{p}_1 - p_1 \rvert \geq \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{2}{\delta}}}{N}} \Big] & \leq \delta 
    \end{split}
\end{equation*}
Therefore, w.p. $\geq 1-\delta$, our sample satisfies 
\begin{equation*}
    \begin{split}
        & \lvert \hat{p}_1 - p_1 \rvert \leq \frac{10}{3} \sqrt{\frac{\sigma^2 \log{\frac{2}{\delta}}}{N}} \\
        \implies & p_1^2 - 2\hat{p}_1 p_1 + \hat{p}_1^2 \leq \frac{100\log{\frac{2}{\delta}}}{9N}(p_1-p_1^2) \triangleq K_{\delta N} (p_1 - p_1^2) \\
        \implies & p_1^2(1 + K_{\delta N}) - (2\hat{p}_1 + K_{\delta N})p_1 + \hat{p}_1^2 = 0
    \end{split}
\end{equation*}
Solving the quadratic gives a conservative $\underline{p}_1$.
\\

\noindent We now compare the right-hand side inside the probability statement to the ratio $\frac{p_1}{K}$. 
\begin{equation*}
    \begin{split}
        \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{2}{\delta}}}{N}} & \leq \frac{p_1}{K} \\
        \implies \frac{100p_1(1-p_1) \log{\frac{2}{\delta}}}{9N} & \leq \frac{p_1^2}{K^2} \\
        \frac{50p_1 \log{\frac{2}{\delta}}}{9N} \leq \frac{100p_1(1-p_1) \log{\frac{2}{\delta}}}{9N} & \leq \frac{p_1^2}{K^2} \\
        \implies \frac{9N}{50p_1\log{\frac{2}{\delta}}} & \geq \frac{K^2}{p_1^2} \\
        \implies \frac{9Np_1}{50\log{\frac{2}{\delta}}} & \geq K^2 \\
        \implies K & \leq \frac{3}{5}\sqrt{\frac{Np_1}{2\log{\frac{2}{\delta}}}} \\
        \text{or } N & \geq \frac{50 K^2 \log{\frac{2}{\delta}}}{9 p_1}
    \end{split}
\end{equation*}
We see that this event implies the previous one, because for any valid $K \geq 1 > \frac{3}{5}$, 
\begin{equation*}
    \frac{50 K^2 \log{\frac{2}{\delta}}}{9p_1} = \frac{25K^2}{9}\big(\frac{2\log{\frac{2}{\delta}}}{p_1}\big) \geq \big(\frac{2\log{\frac{2}{\delta}}}{p_1}\big)
\end{equation*}
This analysis suggests that we can proceed as follows: use $\underline{p}_1$ and solve for $\underline{K}_1$ equating
\begin{equation*}
    N = \frac{50\underline{K}_1^2\log{\frac{2}{\delta}}}{9\underline{p}_1}
\end{equation*}
Then we have that, conditioned on the event that Bernstein holds, 
\begin{equation*}
    N = f(\underline{K}_1, \underline{p}_1, \delta) \geq f(\underline{K}_1, p_1, \delta)
\end{equation*}
and we have then that 
\begin{equation*}
    \begin{split}
        \hat{p}_1 & \leq p_1(1 + \frac{1}{\underline{K}_1}) \\
        \implies p_1 & \geq \frac{\underline{K}_1}{\underline{K}_1 +1} \hat{p}_1 \triangleq \underline{p}_1 \\
        & \geq \hat{p}_1 - \frac{1}{\underline{K}_1 +1} \hat{p}_1 \triangleq \underline{p}_1
    \end{split}
\end{equation*}
\end{proof}

\noindent As an added point, note that this also naturally encompasses the need for information; the expected number of 1-events is $\tilde{n}_1 = \mathbb{E}\big[p_1N\big] \approx 6K^2\log{\frac{2}{\delta}}$. To provide an interpretation: for a fixed confidence level, the number of `hits' needed for ever-finer multiplicative concentration scales with the square of the concentrating factor; for a fixed multiplicative factor, sample complexity grows at the standard $\log{\frac{c}{\delta}}$. For $K = 2$ concentration, we have that approximately 50 instances of Case 1 are needed for 99\% confidence over the sampling. This is slightly worse than the $\approx 30$ samples needed for Gaussian approximation of sample means or conformal prediction methods, but contains high confidence over samples, which the other ones do not. 

\subsection{Cost Function Definition}
Now, we need to specify a cost function that will encode the needed behavior: an overestimate of the conditional failure rates that does not rely on randomness in the sample - unless it holds with high probability over counterfactual samples. \\

\noindent The `naive' or `ideal' cost function - that is, one that has an empirical mean exactly equal to the desired cost function - is:
\begin{equation} \label{IdealCost}
    \hat{C}_\xi(E; \#(S_E), \pi) = (\lambda) \frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1]}{\hat{p}_1} + (1-\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]}{1-\hat{p}_1}
\end{equation}

\noindent However, $\hat{p}_1$ is random across samples in an `unstable' way, which makes it challenging to meaningfully give bounds using this cost function. Instead, we use the fact that $\underline{p}_1$ holds across many samples and the fact that $\lambda$ is fixed and known to rearrange the cost function as follows: 
\begin{equation} \label{ActualCost0}
    \tilde{C}_{\xi, 0} (E; \#(S_E), \pi) = (\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1]}{\underline{p}_1} + (1-\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]}{\underline{p}_0}
\end{equation}
(where $\underline{p}_0$ is calculated much the same as $\underline{p}_1$, but because it is assumed to be greater than or equal to 0.5 it is not the `limiting case' and thus is presented analogously but without formal derivation). 

\noindent Now, we can define some terms that, similar to Equation \ref{ActualCost0}, will hold across many samples: 
\begin{equation} \label{ActualCost}
    \begin{split}
        C_\lambda & \triangleq \frac{\lambda}{\underline{p}_1} + \frac{1-\lambda}{\underline{p}_0} \\
        \tilde{C}_\xi(E; \#(S_E), \pi) & = \frac{1}{C_\lambda}\bigg[ (\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1]}{\underline{p}_1} + (1-\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]}{\underline{p}_0}\bigg] \\
        & = (\lambda')\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1] + (1-\lambda')\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]
    \end{split}
\end{equation}
\das{A note here - we could let $C_\lambda = \max\{\lambda/\underline{p}_1, (1-\lambda)/\underline{p}_0\}$ and bound the costs truly between [0, 1] if that improves things. Then the general form of the cost function is (assuming wlog that $\lambda/\underline{p}_1$ is greater; everything follows mutatis mutandis for the other case)
\begin{equation*}
    C_\xi(E; \#(S_E), \pi) = \mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1] + \lambda'' \mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]
\end{equation*}
where $\lambda'' \in [0, 1]$. 
}
\subsection{Procedure}
Draw a sample $S_E$ of $N$ environments iid from an unknown distribution over environments $\mathbb{P}_\mathcal{E}$, where $E_i \in \mathcal{E}$. \\

\noindent In the case of a single time step classifier, we assume that the sensory input is independent of the policy, conditioned on the environment (i.e. as opposed to the multi-time-step setting, where the actions of the policy may affect subsequent sensory observations). Then we have more directly that the environments $E_i$ induce a sample $S_X$ of $N$ observations $X_i \sim \mathbb{P}_\mathcal{X}$. Note that, because $\mathcal{X}$ is the space of observations, it is reasonable to assume that the learner / designer has a parameterization of $\mathcal{X}$ (i.e. it has chosen the sensor suite), even if it does not know the distribution $\mathbb{P}_\mathcal{X}$ induced on $\mathcal{X}$ from $\mathbb{P}_\mathcal{E}$. \\

\noindent Assuming per usual that the detector policy space of hypotheses is denoted $\mathcal{F}$ and is known to the learner / designer (similarly to $\mathcal{X}$), we restate Equation \ref{OPT} with the alternate cost function: 
\begin{equation} \label{ConditionalOPT}
    \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\tilde{C}_\xi(f, E; S_{E,0}, \pi) \bigg]
\end{equation}
Now, for $p_0$, we can use the fact that $p_0 \geq 0.5$ to note that $\underline{K}_0 \geq \frac{3}{5}\sqrt{\frac{Np_0}{2\log{\frac{2}{\delta}}}}$. From this we see that, like $\underline{p}_1$, we get a bound of 
\begin{equation*}
    p_0 \geq \hat{p}_0 - \frac{1}{\underline{K}_0 + 1} \hat{p}_0
\end{equation*}
where the bound is much tighter, however, because $\underline{K}_0 >> \underline{K}_1$. \\

\noindent To tie everything together, we consider the observed empirical cost vis-a-vis the true conditional probability. Recall Equations \ref{IdealCost}, \ref{ActualCost0}, and \ref{ActualCost}. Substituting, we see that when rescaled by $C_\lambda$, the cost function in Equation \ref{ActualCost} can be bounded as 
\begin{equation*}
    \begin{split}
        \hat{C}_\xi (\cdot) & \leq \tilde{C}_{\xi, 0}(\cdot) \\
        & = C_\lambda \tilde{C}_\xi(E; \#(S_E),\pi) \\
        & = (\lambda) \frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1]}{\frac{\underline{K}_1}{\underline{K}_1 + 1} \hat{p}_1} + (1-\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]}{\frac{\underline{K}_0}{\underline{K}_0 + 1} \hat{p}_0} \\
        & \leq \frac{\underline{K}_1 + 1}{\underline{K}_1} \big[\hat{C}_\xi (\cdot)\big] \\
        \implies \frac{C_\lambda \tilde{C}_\xi(\cdot)}{N} & = (\lambda) \frac{\underline{K}_1 + 1}{\underline{K}_1} \frac{\hat{p}_{0 \cap 1}}{\hat{p}_1} + (1-\lambda) \frac{\underline{K}_0 + 1}{\underline{K}_0} \frac{\hat{p}_{1 \cap 0}}{ \hat{p}_0} \\
        & = (\lambda) \frac{\underline{K}_1 + 1}{\underline{K}_1} \hat{p}_{0 \rvert 1}
        + (1-\lambda)\frac{\underline{K}_0 + 1}{\underline{K}_0} \hat{p}_{1 \rvert 0} \\
        & \leq (\lambda) \frac{\underline{K}_1 + 1}{\underline{K}_1} \hat{p}_{0 \rvert 1}
        + (1-\lambda)\frac{\underline{K}_1 + 1}{\underline{K}_1} \hat{p}_{1 \rvert 0} \\
        & = \frac{\underline{K}_1 + 1}{\underline{K}_1} \big[\frac{\hat{C}_\xi (\cdot)}{N}\big] \\
        & = \big[\frac{\hat{C}_\xi (\cdot)}{N}\big] \big(1 + \frac{1}{\underline{K}_1}\big)
    \end{split}
\end{equation*}

\noindent Summarizing the result in words: we have a framework that, for any iid sample of environments, constructs a cost function that is (1) a probable, approximate (over)estimate of the desired quantity (weighted mixture of conditional probabilities) and (2) converges to the desired quantity at an asymptotically optimal rate in the number of elements $N$ in the training sample ($\mathcal{O}(\frac{1}{\sqrt{N}})$). Unlike the bounds on the joint probabilities, this method also encodes the implicit dependence on the number of each class observed (successes and failures) and provides a smooth trade-off whereby the relative weighting can be adjusted. Finally, it provides a means of ensuring that the cost function is bounded in $[0, 1]$, which interfaces more cleanly with existing PAC-type guarantees (trying to use, say, Equation \ref{IdealCost} or \ref{ActualCost0} would result in very loose bounds on the cost function range, and thus the concentration inequalities would not be tight. Our method allows for concentration of each element in $[0, 1]$ while encoding the structure that the empirical average cost must be in $[0, 1]$ to ensure that the scaling-up doesn't severely overestimate the resulting cost). \\

\noindent As a matter of interpretability, the resulting cost can be bounded via PAC-Bayes in generalization. Then we have an added $\sqrt{N}$ term affixed to the over-estimate. \das{Need to formalize this a bit more precisely}. \\

\noindent Further, the meaning of a given cost is as follows: a naive strategy achieving $\min\{\lambda', 1-\lambda'\}$ is to simply always detect $0$ or $1$ as determined by $\lambda'$. Intuitively, an `ignorant policy' (i.e. a detector randomly picking $0$ or $1$ and using no information from $x_i$) will attain $0.5$ cost. Pushing cost down is akin to bending the ROC curve (in the `good' direction), or equivalently demonstrating the gain from the use of the detector. 

==> Fall21/conditional_probability_clean.tex <==
\section{PAC-Bayes Bound with Conditional Probabilities}

\subsection{Notation}
\subsubsection{Setting Notation}
Let there be a space of environments $\mathcal{E}$, with unknown representation, and a similarly unknown `world distribution' over environments $\mathbb{P}_\mathcal{E}$ \das{assume sufficient measurability, etc}. Let the sensor space be denoted $\mathcal{X}$, with a possibly known representation. Assume a single-time-step setting, and thus assume that $\mathbb{P}_\mathcal{E}$ induces an (unknown) \das{(sufficiently measurable)} distribution $\mathbb{P}_\mathcal{X}$ over sensor measurements. \\

\noindent A function may be (implicitly) conditioned on or parameterized by a fixed quantity; the distinction is denoted with a semi-colon. We can think of this as a kind of `conditional function' akin to a conditional distribution in probability theory. For example, a real-valued function $F$ depending on a quantity $A$ but implicitly conditioned on a (fixed) quantity $b$ may be expressed $F(A; b): \mathcal{A} \mapsto \mathbb{R}$. The example analogy would be the conditional distribution $F_b(a) = p(A=a \rvert B=b) = \frac{F(A=a,B=b)}{\int_\mathcal{A} F(A=a,B=b) d\mu_A}$ of the joint distribution $F(A, B)$. Where it eases exposition, the conditional variable will be included in a subscript of the function, as in $F_b(a)$. 

\subsubsection{PAC-Bayes Notation}
Denote by $S_\mathcal{E}$ a sample of (training) environments drawn i.i.d. from $\mathbb{P}_\mathcal{E}$. Let $N \triangleq \lvert S_\mathcal{E}\rvert$. The space of detector hypotheses is denoted $\mathcal{F}$, and $\mathbb{P}_\mathcal{F}$ is the space of distributions over $\mathcal{F}$. The action (decision) policy for the physical system is denoted $\pi$ and is assumed fixed. \\

\noindent A true label of success or failure is denoted $y_i$, and is induced by a function $y_i = Y_\pi(E_i; \pi): \mathcal{E} \mapsto \{0, 1\}$. A hypothesis maps from the sensor measurement to an estimated label $\hat{y}_i = f_\pi(X_i; \pi): \mathcal{X} \mapsto \{0, 1\}$. For the setting of failure detection, classification is essentially binary; as such, we will wlog define the events $y_i = \{0, 1\}$ to represent the `true' \{success, failure\} of the policy $\pi$ on the environment $E_i$. Analogously, $\hat{y}_i = \{0, 1\}$ will be interpreted to mean the failure detector outputs of \{no warning, warning\}, respectively. \\

\noindent As a matter of shorthand, events will occasionally be represented by unions and intersections; when this is done, the implicit ordering will be $[\hat{y}_i \cap y_i]$. For example, $[1 \cap 0]$ should be understood to mean `the event $\{\hat{y}_i = 1 \cap y_i = 0\}$.' In words, this would denote `the event that the policy actually succeeds but the detector (needlessly) gives a warning.' 

\subsubsection{Statistical Notation}
For (`empirical') functions and quantities derived from the sample $S_\mathcal{E}$, we will use hat-notation, as we do for predictions of the detector. For modified approximation functions, we will use tilde-notation. As with the set notation for $y_i$, the subscripts of $\{0, 1\}$ will refer to the events \{`true' success, `true' failure\}. For example, $n_0$ and $n_1$ will denote the number of successes and failures of action policy $\pi$, respectively, in $S_\mathcal{E}$, where $n_0 + n_1 = N$. Random variables will be assigned capitalized letters. General spaces $\mathcal{U}$ are calligraphic, distributions expressed over a space $\mathcal{U}$ are denoted $\mathbb{P}_\mathcal{U}$. 

\subsection{Problem Setting}

Following from Section \ref{guaranteed}, we want to address the failure detection optimization problem 
\begin{equation} \label{OPT}
\min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}} C_\pi (f; E, \pi)
\end{equation}
where the cost $C_\pi(\cdot)$ encodes a measure of the performance of the failure detector given policy $\pi$. The nominal cost function equates to the empirical mean risk of the detector (the overall probability of misclassification of a new test environment). However, we would like to generalize to the case of minimizing a mixture of the class-conditional probabilities of misclassification. Henceforth, we will assume two classes; however, extension to many-class cases might be of independent interest. \\

\noindent Mathematically, we illustrate this `generalization' idea by noting that misclassification is expressed by the following cost function:
\begin{equation*}
    \begin{split}
        \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}} & \Big[p_{0 \cap 1} + p_{1 \cap 0} \Big] \\
        = & p_1p_{0 \rvert 1} + p_0p_{1 \rvert 0} \\
        = & (\lambda^*) p_{0 \rvert 1} + (1-\lambda^*)p_{1 \rvert 0}
    \end{split}
\end{equation*}
Therefore, misclassification error amounts to minimization of the sum of class-conditional probabilities weighted by the true (but unknown!) probabilities of each event. We would like to `un-fix' $\lambda^*$ to obtain the same cost function for arbitrary $\lambda \in [0, 1]$:
\begin{equation*}
        \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}} (\lambda) p_{0 \rvert 1} + (1-\lambda)p_{1 \rvert 0}
\end{equation*}

\noindent Ideally, we would like to maintain the standard PAC-Bayes type guarantees; however, the conditional probabilities must be estimated from the sample realization of $n_0$ and $n_1$ (number of successes and failures, respectively). In order to encode this into the cost function in an unbiased way, we need to scale the costs by $N/n_0$ and $N/n_1$ (see Equation \ref{NaiveCost}). However, this causes problems in the standard PAC-Bayes analysis for two reasons: first, because the costs are no longer in $[0, 1]$, and second, because $n_0$ and $n_1$ are themselves random variables that depend on the particular sample. \\
\begin{equation} \label{NaiveCost}
\begin{split}
    \hat{C}_\pi(f; E, \pi) & = (\lambda) \frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 0 \cap 1]}{\hat{p}_1} + (1-\lambda)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} 1 \cap 0]}{[1-\hat{p}_1 \triangleq \hat{p}_0]} \\
    \implies \frac{1}{N} \sum_{i=1}^N \hat{C}_\pi(f; E, \pi) & = \lambda \frac{\#(0 \cap 1)}{n_1} + (1-\lambda) \frac{\#(1 \cap 0)}{n_0} \\
    & = \lambda \hat{p}_{0 \rvert 1} + (1-\lambda)\hat{p}_{1 \rvert 0}
    \end{split}
\end{equation}

%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%

\subsection{Initial Setup and Bounding the Success/Failure}
Draw a sample $S_E$ of $N$ environments i.i.d. from some unknown $\mathbb{P}_\mathcal{E}$;  $S_E = \{E_i\}_{i=1}^N \overset{\text{i.i.d.}}{\sim} (\mathbb{P}_\mathcal{E})^N$. Let $S_X$ denote the set of induced feature vectors $x_i$ corresponding to each environment $E_i \in S_E$ over which the algorithm will learn to detect failures. $S_Y$ will denote the set of success and failure labels $\{y_i\}$ induced by the action policy $\pi$. \\

\noindent Let $\hat{p}_i \triangleq n_i/N$ denote the empirical class rates induced by $\pi$ on $S_E$, let $D \in \mathbb{N}$ be the number of classes, and $\hat{\mathbf{p}} \in \Delta_D$ be the vector of $\hat{p}_i$ on the probability simplex. Fix $\mathbf{\lambda} \in \Delta_D$ that denotes the relative importance of misclassification across classes. Given a fixed sample size $N$, fixed $\lambda$, and chosen confidence level $\delta$, we can define underestimates of the probabilities as $\underline{p}_i$. We can use concentration inequalities to give a multiplicative bound whp on the empirical success/failure rates. % From here, assume $D=2$ and wlog $n_1 \leq n_0$.

\begin{lemma}
With probability $\geq 1-\delta$ over samples of size $N$, for any true $\mathbf{p} \in \Delta_D$ and empirical lower bound $\underline{\mathbf{p}} \preceq \Delta_D$, if the following definition for element $K_i$ of $\mathbf{K} \in \mathbb{R}^D$ 
\begin{equation}
    1 < K_i \leq \underline{K}_i \triangleq \frac{3}{5} \bigg[\sqrt{\frac{N \underline{p}_i}{2\log{\frac{D}{\delta}}}}\bigg] = \bigg[\frac{3}{5\sqrt{2\log{\frac{D}{\delta}}}}\bigg] \sqrt{\underline{n}_i}
\end{equation}
can be made valid for all $i \in \{0, ..., D-1\}$, then we have that $\forall i$, $p_i \geq \frac{K_i}{K_i+1} \hat{p}_i = \hat{p}_i - \frac{1}{K_i+1} \hat{p}_i$

%% need a factor of 2 in log to also get this from union bounds: $\hat{p}_i \geq p_i\frac{K_i-1}{K_i}$ and %%
\end{lemma}
\begin{proof}
The result follows from an application of Bernstein's inequality to the empirical mean of iid Bernoulli (multinoulli) random variables. \\

\noindent Fix $i$. From the inequality: 
\begin{equation*}
\begin{split}
    \mathbb{P}\Big[\sum_{i=1}^N X_i - N\mu \geq t \Big] & \leq \text{exp}(\frac{-t^2}{2 \sum \sigma_i^2 + 2t/3}) \triangleq \frac{\delta}{D} \\
    \implies \log{\frac{D}{\delta}} & = \frac{t^2}{2N\sigma^2 + 2t/3} \\
    & \geq \min\{\frac{t^2}{4N\sigma^2}, \frac{3t}{4}\}
    \end{split}
\end{equation*}
This allows us to reason about $t$ as follows: 
\begin{equation*}
    \begin{split}
        \log{\frac{D}{\delta}} & \geq \frac{t^2}{4Np_i(1-p_i)} \\
        \implies t & \leq \sqrt{4Np_i(1-p_i)\log{\frac{D}{\delta}}}\text{, and} \\
        \log{\frac{D}{\delta}} & \geq \frac{3t}{4} \\
        \implies t & \leq \frac{4 \log{\frac{D}{\delta}}}{3}
    \end{split}
\end{equation*}
Therefore, w.p. $\geq 1-\frac{\delta}{D}$, we have that 
\begin{equation*}
    \mathbb{P}\Big[\sum_{i=1}^N X_i - N\mu \geq t \Big] \leq \frac{\delta}{D} 
\end{equation*}
where 
\begin{equation*}
    t = 2\sqrt{N\sigma^2\log{\frac{D}{\delta}}} + \frac{4\log{\frac{D}{\delta}}}{3}
\end{equation*}
And for $N \geq  \frac{\log{\frac{D}{\delta}}}{\sigma^2}$, we have that
\begin{equation*}
    \sqrt{N\sigma^2 \log{\frac{D}{\delta}}} \geq \log{\frac{D}{\delta}}
\end{equation*}
which implies that for $N \geq \frac{\log{\frac{D}{\delta}}}{\sigma^2}$, 
\begin{equation*}
    t \leq \frac{10}{3}\sqrt{N \sigma^2 \log{\frac{D}{\delta}}}
\end{equation*}
Switching to the empirical mean (i.e. dividing by $N$), we have that the Bernstein inequality can be equivalently expressed as: 
\begin{equation} \label{MeanBernstein}
    \mathbb{P}\bigg[\frac{1}{N}\sum_{i=1}^N X_i - \mu \geq \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{D}{\delta}}}{N}} \bigg] \leq \frac{\delta}{D}
\end{equation}
and equivalently, that 
\begin{equation*}
    \mathbb{P}\Big[\hat{p}_i - p_i \geq \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{D}{\delta}}}{N}} \Big] \leq \frac{\delta}{D}
\end{equation*}
Therefore, w.p. $\geq 1-\frac{\delta}{D}$, our sample satisfies 
\begin{equation} \label{Quadratic_Prob}
    \begin{split}
        & \hat{p}_i - p_i \leq \frac{10}{3} \sqrt{\frac{\sigma^2 \log{\frac{D}{\delta}}}{N}} \\
        \implies & p_i^2 - 2\hat{p}_i p_i + \hat{p}_i^2 \leq \bigg[\frac{100\log{\frac{D}{\delta}}}{9N} \triangleq K_{\delta N} \bigg] (p_i-p_i^2)\\
        \implies & p_i^2(1 + K_{\delta N}) - (2\hat{p}_i + K_{\delta N})p_i + \hat{p}_i^2 \leq 0
    \end{split}
\end{equation}
Solving the quadratic with equality to $0$ and taking the lesser solution gives a conservative $\underline{p}_i$. Taking the union over all $D$ classes gets the desired result with probability greater than $1 - \delta$. We now compare the right-hand side inside the probability statement of Equation \ref{MeanBernstein} to the ratio $\frac{p_i}{K_i}$: (we assume $p_i < 0.5$ here)
\begin{equation*}
    \begin{split}
        \frac{10}{3}\sqrt{ \frac{\sigma^2 \log{\frac{D}{\delta}}}{N}} & \leq \frac{p_i}{K_i} \\
        \implies \frac{100p_i(1-p_i) \log{\frac{D}{\delta}}}{9N} & \leq \frac{p_i^2}{K_i^2} \\
        \frac{50p_i \log{\frac{D}{\delta}}}{9N} \leq \frac{100p_i(1-p_i) \log{\frac{D}{\delta}}}{9N} & \leq \frac{p_i^2}{K_i^2} \\
        \implies \frac{9N}{50p_i\log{\frac{D}{\delta}}} & \geq \frac{K_i^2}{p_i^2} \\
        \implies \frac{9Np_i}{50\log{\frac{D}{\delta}}} & \geq K_i^2 \\
        \implies K_i & \leq \frac{3}{5}\sqrt{\frac{Np_i}{2\log{\frac{D}{\delta}}}} \\
        \text{or } N & \geq \frac{50 K_i^2 \log{\frac{D}{\delta}}}{9 p_i}
    \end{split}
\end{equation*}
We see that this event implies the previous one, because for any valid $K_i \geq 1 > \frac{3}{5}$, 
\begin{equation*}
    \frac{50 K_i^2 \log{\frac{D}{\delta}}}{9p_i} = \frac{25K_i^2}{9}\big(\frac{2\log{\frac{D}{\delta}}}{p_i}\big) \geq \big(\frac{2\log{\frac{D}{\delta}}}{p_i}\big)
\end{equation*}
This analysis suggests that we can proceed as follows: use $\underline{p}_i$ and solve for $\underline{K}_i$ by equating
\begin{equation*}
    N = \frac{50\underline{K}_i^2\log{\frac{D}{\delta}}}{9\underline{p}_i}
\end{equation*}
Then we have that, conditioned on the event that Bernstein holds, 
\begin{equation*}
    N = f(\underline{K}_i, \underline{p}_i, \delta) \geq f(\underline{K}_i, p_i, \delta)
\end{equation*}
and we have then that 
\begin{equation*}
    \begin{split}
        \hat{p}_i & \leq p_i(1 + \frac{1}{\underline{K}_i}) \\
        \implies p_i & \geq \frac{\underline{K}_i}{\underline{K}_i +1} \hat{p}_i \triangleq \underline{p}_i \\
        & \geq \hat{p}_i - \frac{1}{\underline{K}_i +1} \hat{p}_i \triangleq \underline{p}_i
    \end{split}
\end{equation*}
\end{proof}


\subsection{Cost Function Definition}
Now, we need to specify a cost function that will encode the needed behavior: an overestimate of the conditional failure rates that does not rely on randomness in the sample - unless it holds with high probability over samples. The `naive' or `ideal' cost function - that is, one that has an empirical mean exactly equal to the desired cost function - is:
\begin{equation} \label{IdealCost}
    \hat{C}_\xi(E; S_E, \pi) = \sum_{d=0}^{D-1} (\lambda_d) \frac{\mathbbm{1}[E \overset{\pi}{\mapsto} \neg d \cap d]}{\hat{p}_d}
\end{equation}

\noindent However, the $\hat{p}_i$ are random across samples in an `unstable' way, which makes it challenging to meaningfully give bounds using this cost function. Instead, we use the fact that $\underline{p}_i$ holds across many samples and the fact that $\lambda$ is fixed and known to rearrange the cost function as follows: 
\begin{equation} \label{ActualCost0clean}
    \tilde{C}_{\xi, 0} (E; S_E, \pi) = \sum_{d=0}^{D-1} (\lambda_d)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} \neg d \cap d]}{\underline{p}_d}
\end{equation}

\noindent Now, we can define some terms that, similar to Equation \ref{ActualCost0clean}, will hold with high probability across training sets: 
\begin{equation} \label{ActualCostclean}
    \begin{split}
        C_\lambda & \triangleq \sum_{d=0}^{D-1}\frac{\lambda_d}{\underline{p}_d} \\
        \tilde{C}_\xi(E; S_E, \pi) & = \frac{1}{C_\lambda}\bigg[ \sum_{d=0}^{D-1} (\lambda_d)\frac{\mathbbm{1}[E \overset{\pi}{\mapsto} \neg d \cap d]}{\underline{p}_d}\bigg] \\
        & = \sum_{d=0}^{D-1} (\lambda'_d)\mathbbm{1}[E \overset{\pi}{\mapsto} \neg d \cap d]
    \end{split}
\end{equation}

\subsection{Procedure}
Draw a sample $S_E$ of $N$ environments iid from an unknown distribution over environments $\mathbb{P}_\mathcal{E}$, where $E_i \in \mathcal{E}$. \\

\noindent In the case of a single time step classifier, we assume that the sensory input is independent of the policy, conditioned on the environment (i.e. as opposed to the multi-time-step setting, where the actions of the policy may affect subsequent sensory observations). Then we have more directly that the environments $E_i$ induce a sample $S_X$ of $N$ observations $X_i \sim \mathbb{P}_\mathcal{X}$. Note that, because $\mathcal{X}$ is the space of observations, it is reasonable to assume that the learner / designer has a parameterization of $\mathcal{X}$ (i.e. it has chosen the sensor suite), even if it does not know the distribution $\mathbb{P}_\mathcal{X}$ induced on $\mathcal{X}$ from $\mathbb{P}_\mathcal{E}$. \\

\noindent Assuming per usual that the detector policy space of hypotheses is denoted $\mathcal{F}$ and is known to the learner / designer (similarly to $\mathcal{X}$), we restate Equation \ref{OPT} with the alternate cost function: 
\begin{equation} \label{ConditionalOPT}
    \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\tilde{C}_\xi(f, E; S_E, \pi) \bigg]
\end{equation}
Now, for any $p_i \geq 0.5$, we note that $\underline{K}_i \geq \frac{3}{5}\sqrt{\frac{Np_i}{2\log{\frac{D}{\delta}}}}$. From this we see that, just like $\underline{p}_j$ for $p_j < 0.5$, we get a bound of 
\begin{equation*}
    p_i \geq \hat{p}_i - \frac{1}{\underline{K}_i + 1} \hat{p}_i
\end{equation*}
where the bound is much tighter, however, because $\underline{K}_i >> \underline{K}_j$. \\

\noindent To tie everything together, we consider the observed empirical cost vis-a-vis the true conditional probability. Recall Equations \ref{IdealCost}, \ref{ActualCost0clean}, and \ref{ActualCostclean}. Substituting, we see that when rescaled by $C_\lambda$, the cost function in Equation \ref{ActualCostclean} can be bounded as 
\begin{equation*}
    \begin{split}
        \hat{C}_\xi (\cdot) & \leq \tilde{C}_{\xi, 0}(\cdot) \\
        & = C_\lambda \tilde{C}_\xi(E; S_E,\pi) \\
        & = \sum_{d=0}^{D-1} (\lambda_d) \frac{\mathbbm{1}[E \overset{\pi}{\mapsto} \neg d \cap d]}{\frac{\underline{K}_d}{\underline{K}_d + 1} \hat{p}_d} \\
        & \leq \frac{\underline{K}_{min} + 1}{\underline{K}_{min}} \big[\hat{C}_\xi (\cdot)\big] \\
        \implies \frac{\sum_{n=1}^N C_\lambda \tilde{C}_\xi(\cdot)}{N} & = \frac{1}{N} \sum_{d=0}^{D-1} \sum_{n=1}^N (\lambda_d) \frac{\underline{K}_d + 1}{\underline{K}_d} \frac{\mathbbm{1}[E_n \overset{\pi}{\mapsto} \neg d \cap d]}{\hat{p}_d} \\
        & = \sum_{d=0}^{D-1} (\lambda_d) \frac{\underline{K}_d + 1}{\underline{K}_d} \frac{\hat{p}_{\neg d \cap d}}{\hat{p}_d} \\
        & = \sum_{d=0}^{D-1} (\lambda_d) \frac{\underline{K}_d + 1}{\underline{K}_d} \hat{p}_{\neg d \rvert d} \\
        & \leq \frac{\underline{K}_{min} + 1}{\underline{K}_{min}} \sum_{d=0}^{D-1} (\lambda_d) \hat{p}_{\neg d \rvert d} \\
        & = \frac{\underline{K}_{min} + 1}{\underline{K}_{min}} \bigg[\frac{\sum_{n=1}^N \hat{C}_\xi (\cdot)}{N}\bigg] \\
        & = \bigg[\frac{\sum_{n=1}^N \hat{C}_\xi (\cdot)}{N}\bigg](1 + \frac{1}{\underline{K}_{min}})
    \end{split}
\end{equation*}

\noindent Summarizing the result in words: we have a framework that, for any iid sample of environments, constructs a cost function that is (1) a probable, approximate (over)estimate of the desired quantity (weighted mixture of conditional probabilities) and (2) converges to the desired quantity at an asymptotically optimal rate in the number of elements $N$ in the training sample ($\mathcal{O}(\frac{1}{\sqrt{N}})$). Unlike the bounds on the joint probabilities, this method also encodes the implicit dependence on the number of each class observed (successes and failures) and provides a smooth trade-off whereby the relative weighting can be adjusted. Finally, it provides a means of ensuring that the cost function is bounded in $[0, 1]$, which interfaces more cleanly with existing PAC-type guarantees (trying to use, say, Equation \ref{IdealCost} or \ref{ActualCost0clean} would result in very loose bounds on the cost function range, and thus the concentration inequalities would not be tight. Our method allows for concentration of each element in $[0, 1]$ while encoding the structure that the empirical average cost must be in $[0, 1]$ to ensure that the scaling-up doesn't severely overestimate the resulting cost). \\

\noindent As a matter of interpretability, the resulting cost can be bounded via PAC-Bayes in generalization. Then we have an added $\sqrt{N}$ term affixed to the over-estimate. \das{Need to formalize this a bit more precisely}. \\

\noindent Further, the meaning of a given cost is as follows: a naive strategy achieving $\min\{\lambda', 1-\lambda'\}$ is to simply always detect $0$ or $1$ as determined by $\lambda'$. Intuitively, an `ignorant policy' (i.e. a detector randomly picking $0$ or $1$ and using no information from $x_i$) will attain $0.5$ cost. Pushing cost down is akin to bending the ROC curve (in the `good' direction), or equivalently demonstrating the gain from the use of the detector. 

\newpage{}
\subsection{Procedure [FULL]}
Draw a sample $S_E$ of $N$ environments iid from an unknown distribution over environments $\mathbb{P}_\mathcal{E}$, where $E_i \in \mathcal{E}$. Choose a confidence level $\delta \in (0, 1)$. \\

\noindent The environments $E_i \in S_E$ induce a sample $S_X$ of $N$ sensor observations $X_i \sim \mathbb{P}_\mathcal{X}$. Note that, because $\mathcal{X}$ is the space of observations, we assume that the learner has a parameterization of $\mathcal{X}$ (i.e. it has chosen or has knowledge of the sensor suite), even if it does not know the distribution $\mathbb{P}_\mathcal{X}$ induced on $\mathcal{X}$ by $\mathbb{P}_\mathcal{E}$. \\

\noindent Assuming per usual that the detector policy space of hypotheses is denoted $\mathcal{F}$ and is known to the learner (like $\mathcal{X}$), we restate Equation \ref{OPT} with the alternate cost function: 
\begin{equation} \label{ConditionalOPT_Full}
    \min_{\mathbb{P}_\mathcal{F}} \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\tilde{C}_\xi(f, E; S_E, \pi) \bigg]
\end{equation}

\subsubsection{Necessary Quantities}
Determine $n_s$ and $n_f$, the number of successes and failures in the sample, where $n_s + n_f = N$. Define $\hat{p}_s \triangleq n_s/N$, and $\hat{p}_f \triangleq n_f/N := 1-\hat{p}_s$. Solve for $\underline{p}_s$ and $\underline{p}_f$ via Equation \ref{Quadratic_Prob}. Solve for $\underline{K}_s$, $\underline{K}_f$ via Equation \ref{Underline_K}:
\begin{equation} \label{Underline_K}
\underline{K}_d = \frac{\underline{p}_d}{\hat{p}_d - \underline{p}_d}
\end{equation}

\noindent Calculate $C_\lambda$ via Equation \ref{ActualCostclean}, and define $\tilde{C}_\xi(\cdot, E; S_E, \pi)$ using this $C_\lambda$. 

\subsubsection{Further Steps}
Apply the standard PAC-Bayes design approach. That is, choose a prior over distributions $\mathbb{P}_{\mathcal{F},0}$, train the distribution according to standard global optimization methods, and apply the additive PAC-Bayes bound. This yields (something like):
\begin{equation} \label{FinalVersion_0}
    \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\tilde{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] \leq \frac{1}{N} \sum_{i=1}^N \tilde{C}_\xi(f, E_i \in S_E; \pi) + \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}} 
\end{equation}
Rescaling by $C_\lambda$, we attain: 
\begin{equation}
    \begin{split}
        \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\hat{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] & \leq \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[C_\lambda \tilde{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] \\
        & \leq \frac{C_\lambda}{N} \sum_{i=1}^N \tilde{C}_\xi(f, E_i \in S_E; \pi) + C_
    \lambda \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}} \\
    & \leq \frac{1}{N} \sum_{i=1}^N \hat{C}_\xi(f, E_i \in S_E; \pi)(1 + \frac{1}{\underline{K}_{min}}) + C_
    \lambda \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}} 
    \end{split}
\end{equation}
Without loss of generality, we will assume that the policy has more successes than failures. Further, we note that the weighted sum of conditional probabilities is bounded on $[0,1]$ with probability 1, which means that the desired result is found as:
\begin{equation}
    \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\hat{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] \leq \frac{1}{N} \sum_{i=1}^N \hat{C}_\xi(f, E_i \in S_E; \pi) + \frac{1}{\underline{K}_{f}} + C_
    \lambda \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}}
\end{equation}
And using the following identity:
\begin{equation}
    \begin{split}
        \frac{K_f^2}{p_f^2} & = \frac{9N}{100p_f(1-p_f) \log{\frac{D}{\delta}}}  \\
        \implies K_f^2 & = \frac{9Np_f}{100(1-p_f) \log{\frac{D}{\delta}}} \\
        \implies K_f & \geq \frac{3}{10} \sqrt{\frac{N\underline{p}_f}{(1-\underline{p}_f)\log{\frac{2}{\delta}}}} \triangleq \underline{K}_f 
    \end{split}
\end{equation}
we see that the result can be reduced to
\begin{equation}
    \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\hat{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] \leq \frac{1}{N} \sum_{i=1}^N \hat{C}_\xi(f, E_i \in S_E; \pi) + \frac{10}{3} \sqrt{\frac{(1-\underline{p}_f)\log{\frac{2}{\delta}}}{N\underline{p}_f}} + C_
    \lambda \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}}
\end{equation}
Finally, noting that there exists a deterministic strategy of always guessing the class $d$ with lowest $\lambda'_d$, we see that for $D$ classes, the empirical cost can always be made smaller than $\min_d \lambda'_d \leq \frac{1}{D}$. Assuming that we will improve upon this strategy, we can wlog assume that the empirical cost is less than $\frac{1}{D}$ and thus scale the second term by $\frac{1}{D}$, achieving 
\begin{equation}
    \underset{E \sim \mathbb{P}_\mathcal{E}}{\mathbb{E}} \underset{f \sim \mathbb{P}_\mathcal{F}}{\mathbb{E}}\bigg[\hat{C}_\xi(\cdot, \cdot; S_E, \pi) \bigg] \leq \frac{1}{N} \sum_{i=1}^N \hat{C}_\xi(f, E_i \in S_E; \pi) + \frac{10}{3D} \sqrt{\frac{(1-\underline{p}_f)\log{\frac{2}{\delta}}}{N\underline{p}_f}} + C_
    \lambda \sqrt{\frac{\mathbb{D}_{KL}(\mathbb{P}_\mathcal{F} \rVert \mathbb{P}_{\mathcal{F},0}) + \log{\frac{2\sqrt{N}}{\delta}}}{2N}}
\end{equation}

==> Fall21/failure_detection.tex <==

\section{Guaranteed Failure Detection} \label{guaranteed}
Fix a policy $\pi$ which performs a particular task in environments $E \sim \D$. Let a rollout function map policy $\pi$ and an environment $E$ to a set of positions $\{x_1, x_2, \dots, x_T\}$ within the environment. We want the failure detector to continuously monitor for the possibility of a failure while the policy is performing the task. Thus, consider a failure detector $f$ which takes as input the history of sensor measurements up until the current time step. Let $f$ output a binary value where $0$ indicates a prediction of success and $1$ indicates a prediction of failure. Then, at any time step, we can compute the failure detector's output. Let cost function for the failure detector $C_\pi(f; E)$ on environment $E$ be defined as follows: a cost of $0$ is incurred if the failure predictor predicts any failure prior to the occurrence of the failure, or if the predictor never says there is a failure and there isn't one. We assign $C = 1$ otherwise (i.e. $f$ predicts a failure after the failure happens, predicts failure when there isn't one, doesn't predict a failure when there is one). 

We will learn a distribution over failure detectors $F$ (so that we can use the PAC-Bayes framework) with the following objective:
\begin{equation}
    \min_{F} \underset{E \sim \D}{\EE} \underset{f \sim F}{\EE} C_\pi(f; E)
\end{equation}

Suppose we are given a dataset $S\sim \D^n$ for training. We can then write the following PAC-Bayes guarantee (which holds for any $F$ with probability $1 - \delta$ over a sampling of $S \sim \D^n$).  
% (Note that the cost is assigned for an entire trajectory and thus we don't have independence issues with data within-rollout).
\begin{equation}
        \underset{E \sim \D}{\EE} \ \underset{f \sim F}{\EE} \ C_\pi(f; E) \leq \sum_{i=1}^{n} \underset{f \sim F}{\EE} \ C_\pi(f; E_i) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{equation}

In training, we find an $F$ and try to minimize the upper bound (i.e. by taking gradient steps, evolutionary strategies, or setting up and solving relative entropy programs) to provide a tight bound on the expected $\EE_{f \sim F} C_\pi(f; E)$. This corresponds to the probability that the detector will be \emph{incorrect} about what the policy will do. Thus, we achieved the form of the guarantee we were aiming for: on a new environment, we have a $(1 - \text{[upper bound]})$ probability of successfully detecting whether or not there will be a failure. 
% \alec{Switch to standard PAC-Bayes bound, don't need derandomized version.} I think that the derandomized PAC-Bayes bound makes sense here since we need to evaluate $\EE_{f\sim F} C_\pi(f; E)$ for a new environment $E$ in order to determine if there was a failure. It would be impractical to assume we can run multiple times if there is a high cost of failure. Thus, we can write following derandomized PAC-Bayes bound (which holds for any $F$ with probability $1 - \delta$ over a sampling of $S \sim \D^n$ and $f \sim F$):
% \begin{equation} \label{eq:fd loss pointwise bound}
%         \underset{E \sim \D}{\EE} \ C_\pi(f; E) \leq \sum_{i=1}^{n} \ C_\pi(f; E_i) + \sqrt{\frac{D_2(F \| F_0) + \ln\frac{2\sqrt{n}}{(\delta/2)^3}}{2n}}
% \end{equation}
% (Note: here we have set $\alpha = 2$ for the Renyi divergence $D_\alpha$.)

\subsection{Decoupling the Detector's Loss}
In our setup, a cost of $0$ is achieved if the failure detector is \emph{correct}, not just if a failure was going to occur and the detector predicted the event. Consider the following example: the failure detector always says there will be a failure. Then, deploying the conservative policy will prevent failures in all test environments; however, it will also always prevent robot from completing the task. Thus it would be interesting to study the improved effectiveness of the policy including the failure detector and conservative policy. % We will say the failure detector is perfect if the conservative policy is only deployed when a crash was going to occur. This ensures the maximum number of tasks are completed while completely avoiding failures. 

% Given the training data $S$, we can estimate the probability that the policy will fail running the standard policy $\pi$ while allowing for failures, but noting if the failure detector indicated the occurrence of a failure. 
Let $p$ be the probability that policy $\pi$ fails on $\D$, and $\widehat{p}$ be the probability that policy $\pi$ fails on $S$. A false positive (fp) corresponds to the detector indicating a failure when the policy did not fail. A false negative (fn) indicates a failure from the policy but no detection. A perfect detector will have a 0 fp and fn rate are 0. Let the probability of a fp and fn be $p_{\text{fp}}$ and $p_{\text{fn}}$ respectively. We then have probabilities for the 4 cases (assuming the conservative policy stops the task and -- no failure occurs but the task is not completed). Let FD be the failure detector.
\begin{enumerate}
    \item The FD is too conservative -- the policy would have succeeded but the FD guesses that a failure will occur: $p_{\text{fp}}$
    \item The FD is correct about no failure occurring: $1 - p - p_{\text{fp}}$ 
    \item The FD is correct that a crash will occur, and saves the policy from failing: $p - p_{\text{fn}} $
    \item The FD misses a policy failure: $p_{\text{fn}}$
\end{enumerate}
Here the cost we wrote above is Case 1 + Case 4 or $p_{\text{fp}} + p_{\text{fn}}$, i.e., when the failure detector is incorrect about when a failure or success occurs. Are there ways to provide guarantees on any of the other quantities? $p_{\text{fn}}$ is of particular interest because it can represent the probability of failure when we use the failure detector in practice. However it's important to not allow the detector to become too conservative. Thus I think it makes sense to train with the case 1 + case 4 loss and then compute bounds for whichever thing we are interested. 

% Suppose we split our training dataset into two sets. $S_f$ is the set of environments on which the policy will fail, $S_s$ is the set of environments on which the policy will succeed. Note that $|S_f| = |S|*\widehat{p}$. \begin{equation}
%     \widehat{p}_{\text{fn}} \text{ (empirically on }S_f) =\frac{1}{n}\sum_{E \in S_f} C_{\pi}(f; E)
% \end{equation}
% and 
% \begin{equation}
%     \widehat{p}_{\text{fp}} \text{ (empirically on }S_s)=\frac{1}{n} \sum_{E \in S_s}C_{\pi}(f; E).
% \end{equation}
We can compute a PAC-Bayes bound on either of these quantities and bound the false-negative and false-positive rate directly. Let $C^{\text{fn}}_\pi(f;E)$ be the cost which assigns a $1$ only when Case 4 occurs (i.e. a false-negative occurs). Thus $p_{\text{fn}} = \EE_{E\sim \D}C^{\text{fn}}_\pi(f;E)$. Then with high probability over a sampling of $S \sim \D$:
\begin{equation}
        p_{\text{fn}} = \underset{E \sim \D}{\EE}  C^{\text{fn}}_\pi(f; E) \leq  \underbrace{\frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E)}_{\widehat{p}_{\text{fn}}} + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{equation}

\das{Just wanted to add a comment about some possible additional quantities of interest. Specifically, I wonder if there might be some value in also considering the conditional probabilities. Something like $p_{n\rvert f}$ (the probability of a negative result given failure) might be relatable in some way to existing learning or statistical mechanisms. Such a quantity will almost certainly be dependent on the much smaller quantity $n_f$ (rather than the total number of samples); however, it seems to represent more fully the `gain' of the detector. Using the unconditioned $p_{nf}$ is of course fundamentally the same (just scaled down by the true expected fraction of failures over the distribution). I don't have a sense, though, of whether the bounds are sensitive to this.} \\

\das{Additionally, the practical use of the detector might be demonstrated effectively by an ROC-like curve of $p_{n \rvert f}$ vs $p_{p \rvert s}$. When there are no false negatives, we expect that the algorithm is just always guessing failure and thus the rate of false positives should be high. Similarly, with many false negatives, we would (hope) that at least the false positives should be low. But if the curve `bends in the right direction' it would suggest that more false negatives can be eliminated without sacrificing as much.}


We can try to get a bound on the probability of a false positive, conditioned on an environment causing a failure, since it may be scaled more appropriately than $p_{\text{fn}}$. Starting with the bound on $p_{\text{fn}}$ which holds with high probability over a sampling of $S \sim \D$
\begin{align}
        \underset{E \sim \D}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}} \\ \underbrace{p_s\underset{E \sim \D_s}{\EE}  C^{\text{fn}}_\pi(f; E)}_{=0} + p_f\underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}} \\
        p_f\underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S_f} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{align}
However we do not know $p_f$ so we lower bound it by $\bar{p}_f$ with probability $1-\delta'$. With a union bound we can say the following with probability at least $1 - \delta' - \delta$ over a sampling of $S \sim \D^n$:
\begin{equation}
    \underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) \leq  \frac{1}{\bar{p}_f n} \sum_{E\in S_f} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \frac{1}{\bar{p}_f}\sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{equation}
Now let's bound $p_f$ with a standard concentration inequality: \alec{I think this is right but will check}
\begin{align}
    P\big[p_f \geq \widehat{p}_f - t \big] \geq 1 - e^{-2nt^2}  \\
    P\Bigg[p_f \geq \underbrace{\widehat{p}_f - \sqrt{\frac{\ln(\frac{1}{\delta'})}{2n}}}_{\bar{p}_f} \Bigg] \geq 1 - \delta'
\end{align}
However, if $\widehat{p}_f - \sqrt{\frac{\ln(\frac{1}{\delta'})}{2n}} \leq 0$, then our guarantee is vacuous! Thus, this will not work for very small $p_f$. 
\alec{@David, I think you're right that we probably can't do any better than this. It would be weird if we could avoid a second $\delta$ and a union bound all together. If things were conditioned on the distribution over the failure detector (instead of the distribution over samples) we could use the a data-processing inequality and not need a union bound (which is more like what I did in the PAC-BUS paper)... as it stands I still think this is cool, perhaps useful even though we compute it by directly loosening the bound on the false-negative rate.}

==> Fall21/median_convergence.tex <==
\section{Example: Convergence of the Sample Median}
For reference, Algorithm 1 from \cite{luo_sample-efficient_2021} is reproduced here. \\
\begin{figure}[!htbp]
    \centering
    \includegraphics{images/Conformal_Alg1.png}
    \caption{Algorithm 1 from \cite{luo_sample-efficient_2021}}
    \label{Base_Alg}
\end{figure}

\iffalse 
\noindent Consider the case where every sample in the training set is a failure (for simplicity). Choose $\epsilon = 0.5$, and assume that $p(g(Y) \rvert \text{ failure }) = p(g(Y)) = \mathcal{U}(0, 1)$. Then with probability 1, the algorithm will set $U = 0$ (i.e. wp 1, $g(Y_t)$ are distinct for all $t \in \{1, 2, ..., T, T+1\}$) and thus line 3 of Algorithm \ref{Base_Alg} sets $U = 0$). Let $\mathcal{A}_<$ denote the set in the numerator of $q$ in line 4. That is, it is the set of failures with a surrogate score less than the surrogate score of the test point $(\hat{Y},\hat{Z})$. \\
\fi 

\noindent Precisely: let $Y_t \sim \mathcal{U}(0,1)$. Let $Z_t = Y_t$, and let $f, g: [0,1] \mapsto [0,1]$ be the identity functions. That is, for all $x \in [0, 1]$, $f(x) = g(x) = x$. Let $f_0 = 2$. \\

\noindent Then we have that every sample is a failure, and $p(g(Y)) = p(Y) = \mathcal{U}(0,1)$. As such, with high probability every sample point is distinct and $U = 0$ on line three of Algorithm \ref{Base_Alg}. Denoting $\{a \in \mathcal{A} \rvert a < g(\hat{Y})\}$ as $A_<$, we observe the following:

\begin{equation}
\begin{split}
    \lvert \mathcal{A} \rvert & = T \text{;} \\
    q & = \frac{\lvert \mathcal{A}_{<} \rvert + 1}{\lvert \mathcal{A} \rvert + 1} \\
    & \geq \frac{\lvert \mathcal{A}_{<} \rvert}{\lvert \mathcal{A} \rvert} \triangleq \bar{q} \\
    & \geq 1-\epsilon \\
    \end{split} 
\end{equation}

We note that at least one of the two distinct $\geq$ must hold with strict inequality, for any $\epsilon > 0$. That is, either $1 > q > \bar{q} \geq (1-\epsilon)$ or $1 = q = \bar{q} > 1-\epsilon$. As such, $\bar{q} \geq 1-\epsilon \implies q > 1-\epsilon$, i.e. is a sufficient condition for a false negative. \\

Continuing, we note that this result is precisely a quantile selector; choosing $\epsilon = 0.5$, we see that $\bar{q} \geq 1-\epsilon \iff \hat{Y} \geq \text{median}(S_T)$. \\

From this, we conclude that, in order for the Algorithm to be $\epsilon + \frac{1}{T}$ safe w.p. 1, it must be the case that $m_T > 1 - \epsilon - \frac{1}{T}$ with probability 1, which is not true (it converges whp at $\frac{1}{\sqrt{T}}$ in the asymptotic limit). Which suggests to me that the conformal prediction result is a result in expectation, and not one that holds with (arbitrarily) high probability (i.e. a PAC-like guarantee). Further, $\epsilon = 0.5$ is selected so that the median can be discussed; in general, the same analysis should(?) hold for convergence of any sample quantile (perhaps up to some scaling factors, etc). \\

\sush{I don't think we need the median to converge to the ``true" median for their argument to hold. The proof relies on the fact that all $(Y,Z)$ are identically distributed (exchangeability$\implies$identical). If they are identical, then the rank of $(\hat{Y},\hat{Z})$ --- as ordered by the surrogate score --- is uniformly distributed. Another way to see the uniformity is that all permutations of the training + test data are equally likely. This uniform distribution is the source of the $1/T$ term} \\

\das{To Sushant's point, the analogy I would use is the following: imagine a self-driving car rental service that has a parking lot of $N$ cars, each of which armed with training sample $S_n$ of $T$ data points. The conformal prediction statement in the paper is correct when you approach the desk clerk and ask to rent a car; i.e. in expectation over *both* the choice of car and new test point, with probability $1 - \epsilon - 1/T$ you will be safe on a single new test point. However, \textit{once you choose a particular car from the lot}, this is no longer necessarily true. Their result is in expectation over the training samples, i.e. over all of the cars in the lot, in addition to over the test point. It does not hold w.h.p. over the choice of car. If we read it as holding either w.p. 1 or w.h.p. over the choice of car, then the sample convergence of the median issue above applies. If it only means in expectation over samples, the above median convergence example is irrelevant. As a comparison, as far as I understand it, our standard PAC-Bayes framework would say that w.h.p. the particular car you select will be $1-\epsilon - 1/T$ safe.} \\

\das{Further, there are existing PAC-Bayes results that appear to achieve this same $\tilde{\mathcal{O}}(1/T)$ rate in expectation (rather than w.h.p.) - see for example \cite{audibert_fast_2009,dalalyan_aggregation_2008, dalalyan_aggregation_2007, van_erven_fast_2015} (these are taken from the comment in \cite{guedj_primer_2019}, from the end of page 13 to the top of page 14, right before section 5.} \\

\noindent As an idea to flesh out what Sushant, Allen, and I discussed on Oct 27 -- consider the relatively general exposition of the problem as follows. \\

\noindent Assume $Y_t \sim \mathcal{D}$ drawn from a distribution with absolutely continuous cdf, and assume a perfect simulator ($Y_t = Z_t$). Assume for convenience that the support of $Y_t$ is bounded w.p. 1 on $[a, b]$. Wlog we bound it on $[a=0, b=1]$. (assuming an unbounded support complicates the analysis, but should not fundamentally change the results). Let $f$ be the identity function, and set $f_0$ to be sufficiently large as to ensure that all samples are failures w.p. 1. Concretely, set $f_0 > b$. This is again wlog, because the desired guarantee conditions on the test case being a failure; in a sense, all of the non-failure cases are irrelevant and we can just set all of the data to be failures. \\

\noindent At this point, we proceed to analyze the algorithm performance. First, by the continuity assumption on the distribution over $Y_t$, $U=0$ with probability 1 (this is the only reason to assume the continuous cdf). Second, we fix $\epsilon \in (0, 1)$ (arbitrarily). Let $q_z: \mathcal{D}^T \mapsto [a, b]$ denote a value on the support of $\mathcal{D}$ corresponding to the empirical z-quantile for a sample $S_T$ of size $T$; that is, the finite-data empirical cdf $\hat{F}(S_T)$ approximating $\mathcal{D}$ has $\hat{F}(q_z) = z$. Now, let the functions $g$, $\bar{g}$ be defined as follows:

\begin{equation*}
    \begin{split}
        g(Y_T, \hat{Y}) & = q_{1-\epsilon}(Y_T) - \hat{Y} \\
        \bar{g}(Y_T, \hat{Y}) & = \mathbbm{1}\Big[g(Y_T,\hat{Y}) > 0 \Big]
    \end{split}
\end{equation*}

We begin an analysis of several possible `guaranteed quantities.' First, we analyze the probability of safety over all of the randomness in the procedure: 

\begin{equation*}
    \begin{split}
        & \mathbb{P}_{\substack{(Y_T,\hat{Y})\sim \mathcal{D}^{T+1}}} \Big[ g(Y_T,\hat{Y}) > 0 \Big] \\
        = & \mathbb{E}_{\substack{(Y_T,\hat{Y})\sim \mathcal{D}^{T+1}}} \Big[ \bar{g}(Y_T, \hat{Y}) \Big]
    \end{split}
\end{equation*}
Now, by the assumption of (`pairwise') independence between the randomness in $Y_T$ and $\hat{Y}$ (i.e. independence for each datum implies pairwise independence, but I think all we technically need is pairwise independence between the data in $Y_T$ and $\hat{Y}$), we can break the joint distribution in $Y_T, \hat{Y}$ into the product of two marginal distributions, which allows us \das{(I think, but haven't included the details here for brevity)} to do the following, via a kind of iterated expectation argument: 
\begin{equation*}
    \begin{split}
     & \mathbb{E}_{\substack{(Y_T,\hat{Y})\sim \mathcal{D}^{T+1}}} \Big[ \bar{g}(Y_T, \hat{Y}) \Big] \\
     = & \mathbb{E}_{\substack{Y_T\sim \mathcal{D}^{T}}} \Big[ \mathbb{E}_{\hat{Y} \sim \mathcal{D}} \big[ \bar{g}(Y_T, \hat{Y}) \rvert Y_T=y_T \big] \Big] \\
     = & \mathbb{E}_{\substack{Y_T\sim \mathcal{D}^{T}}} \Big[x : q_x(\mathcal{D}^T) = q_{1-\epsilon}(Y_T) \Big] \\
     \geq & 1-\epsilon-\frac{1}{T} \\
     \triangleq & 1-\epsilon^*
    \end{split}
\end{equation*}
where the $1/T$ term comes from the discretization error in the empirical density. \\

\noindent In words, I would interpret this guarantee as saying the following: the probability of warning failure, in \textbf{expectation over the entire training pipeline}, is less than $\epsilon^*$ \textbf{for one unsafe situation}. \\

In a very simple sense, imagine the following case: w.p. $\{(1-\epsilon), \epsilon\}$ over training datasets, the resulting decision rule is 100\% safe or 0\% safe. By conformal prediction, it is true that the algorithm, before observing a particular training dataset, is $(1-\epsilon)$-safe on a single test point. However, $\epsilon$ of the time, the resulting decision rule is wrong on every single resulting test point; in general, we may prefer having all of the decision rules be $(1-\epsilon)$-safe than having an $\epsilon$-fraction of `homicidal chauffeur'-like agents. \\

\noindent Now, we consider two alternative meanings of the guarantee, and show that they cannot be the proper understanding. \\

\noindent The second overall (and first `false') case will claim, for any $\epsilon \in (0, 1), T \in \mathbb{N}$, that w.p. 1 over training datasets the expected success rate is greater than $1 - \epsilon - 1/T$. This is false. Wlog choose $\delta > 0$ and a combination of $\epsilon, T$ such that $1-\epsilon-1/T > \delta$. Then w.p. greater than $\delta^T$, the training sample will have every element less than $q_\delta$, and therefore have a success probability in testing less than $\delta$, which is less than $1-\epsilon - 1/T$ by definition. \\

\noindent As a small note to the above, note that for any valid, fixed $\epsilon$, we can choose e.g. $T > \frac{3}{1-\epsilon}$ and $\delta = \frac{1-\epsilon}{2}$ to obtain a valid set. \\

\noindent The third overall (and second `false') case is the most subtle. Assume now that instead of w.p. 1 as in case 2, we simply have that w.h.p. the result is true. This is where we need to use established results on the concentration of sample quantiles to argue that the implication ($1/T$ convergence) is too strong even at `only' whp instead of almost surely. That is where the sample convergence of the median result is used. \\

\noindent For these reasons, it seems that the conformal prediction guarantee must be applied before seeing the training dataset, and thus is in some sense `in expectation' over the training samples. As a reinforcement of this, see the definitions of marginal and conditional coverage (Section 1.1) and distribution-free conditional coverage (Section 2.2) \href{https://www.stat.cmu.edu/~ryantibs/papers/limits.pdf}{here}. (The former on page 456, equations 1.1 and 1.2; the latter on page 459). Essentially, the false cases are a kind of conditional-coverage, whereas the statement I think they are making is in marginal coverage, which is weaker \das{(thank you Allen for pointing out this source)}.



==> Fall21/problem_setup.tex <==
\section{Problem Setup}

Consider an MAV which must avoid obstacles. Suppose the MAV moves according to some fixed policy $\pi$. However, assume that in testing, the cost of a crash is very high because the MAV is expensive or it may damage the object it crashes into. We will use PAC-Bayes bounds on a failure detector and a conservative policy (for the MAV this could be stopping immediately, or moving much more slowly) to guarantee that the probability of failure on test environments is small. 

We assume the standard policy learning setting where environments $E$ are drawn from an underlying distribution over environments $\D$. We don't assume any knowledge of or structure on $\D$, and only have access to the distribution via samples $E \sim \D$. At test time, we must perform (and avoid failure) in new environments drawn from $\D$ given a policy $\pi$. However, note that policy $\pi$ may not necessarily be good, we will still guarantee a low probability of failure. We aim to achieve a guarantee of the following form: with high probability, on a new environment, we have a $.95$ probability of successfully detecting whether or not there will be a failure. If we do detect there will be a failure, we can switch to a conservative policy and avoid failure. This guarantees (with high probability) that there won't be more than $5\%$ failures. However in practice it may be much lower if the failure detector is good at distinguishing between cases where the will and will not fail. I discuss this in a later section.


==> deprecated/conformal_prediction.tex <==
\section{Questions About Conformal Prediction Guarantee}

My primary thoughts on trying to understand the meaning of the guarantees made in \cite{luo_sample-efficient_2021} concern a motivating `counter' example. That is, my understanding of their guarantees runs into issues assimilating this example, and I definitely would value hearing others' thoughts on this case. If I had to try to guess what seems odd, it's that it seems that there is one concentration inequality (that I'm) missing for a more natural interpretation of their result? \\

\noindent Anyway... on to the thing that I am struggling to understand. \\

\noindent Assume the data is i.i.d., that is $(Y,Z) \sim \mathcal{D}$, and assume that $g: \mathcal{Y} \mapsto [0, 1]$, $f: \mathcal{Z} \mapsto [0,1]$. Define the variable $F: \mathcal{Z} \mapsto \{0, 1\}$ to denote the event that the true trajectory fails or succeeds. Specifically, $F(Z) = \mathbbm{1}\big[f(Z) >= f_0\big]$. 

\noindent Then, as I understand it, the safety definition (Definition 1) is equivalent to 
\begin{equation}
    P(w(Y)=1 \rvert F=0) \geq 1-\epsilon
\end{equation}
Note that this is not a probabilistic guarantee (i.e. it doesn't only hold with probability $1-\delta$). I understand it to implicitly hold in expectation over the pair $(Y,Z)$, but maybe this is not accurate. However, in the case that it is meant to hold in expectation over $(Y,Z) \sim \mathcal{D}$, it seems that there is a fundamental tension arising because of the concentration of the sample to the `true' distribution. \\

\noindent Specifically, for i.i.d. data, we can define $p_g(g'): [0,1] \mapsto \mathbb{R}^+$ that describes the distribution over $g' \in [0, 1]$ of surrogate scores attained by samples $(Y,Z) \sim \mathcal{D}$ the true underlying distribution. Now, define $p_{g,f}(g')$ to be the distribution of surrogate scores conditioned on failure, i.e. $P(g \rvert F=0)$. We might intuitively imagine that such a conditional mean likely decreases, etc, to get a sense of how this distribution compares to $p_g(g')$. \\

\noindent Now, imagine that we want to use Algorithm 1 to guarantee $\epsilon$-safety. Assuming that the conditional density is absolutely continuous (I have to imagine such an example exists, and the paper doesn't put any restrictions on $g$ and $f$), we note that with probability 1, no two trajectories $(Y, Y')$ will yield the same surrogate cost, i.e. $g(Y) \neq g(Y')$ w.p. 1. Therefore, considering Algorithm 1, we see immediately that U = 0, and can be ignored. From the i.i.d. assumption, we take as an example the following case: with probability (1-2$\epsilon$), a given, \emph{failing} training point $(Y^*_t, Z^*_t)$ will attain a value $g(Y^*_t) < Q_{1-2\epsilon}$. From independence, it follows that w.p. $(1-2\epsilon)^{\lvert \mathcal{A}\rvert}$, \emph{\textbf{every}} failing data point will lie below the $(1-2\epsilon)$ quantile $Q_{1-2\epsilon}$. \\

\noindent Then it seems to me that $\epsilon$-safety fails with non-trivial probability. That is, conditioned on the `unfortunate' training data, w.p. $2\epsilon$, a randomly drawn new failing trajectory $(Y'_f, Z'_f)$ will lie above the $Q_{1-2\epsilon}$ quantile, and thus line 4 of the Algorithm sets $q = 1$, and returns 0. \\

\noindent I interpret this to mean that, for some `bad' (but i.i.d., albeit unlikely!) draws of training data, the algorithm fails(?) And as such, I don't see how they escape having a probabilistic component. Or at least, it seems unclear how this could hold uniformly across dataset draws, and thus it seems that you either need a probabilistic addition (a la PAC(-Bayes) Learning) or an additional concentration on the iid convergence of the data to its true distribution... \\

\noindent In short, the intuition for my question is that the empirical data $\{(Y_t, Z_t)\}_{t=1}^T$, and in particular the failure cases, need not perfectly match the true distribution except in the large-sample limit(?) In short, their guarantee is with respect to the `true distribution,' while their algorithm is working with the empirical sample, and they only seem to account for the difference with an $\mathcal{O}(1/T)$ term, which surprises me. \\

\noindent Anyway, hopefully this might be useful to others in clarifying the understanding of the problem (and in clarifying my own, pending other comments!)

%%% Concrete Example
\newpage{}
\section{Concrete Example}
Assume that there is a true distribution $\mathcal{D}$ over samples $(Y,Z)$ inducing a distribution over surrogate costs for any surrogate cost function $g$. This true distribution $\mathcal{D}$ returns failing samples with probability $\epsilon_\mathcal{D} = 0.25$ (the 0.25 is WLOG). For completeness we let $f$ be the zero-one failure-success indicator. Let's consider the case where $g$ is actually perfectly separating; we define the density of $g(Y)$ and the conditional densities of $g(Y) \rvert f=\{0,1\}$ as follows:
\begin{equation}
    \begin{split}
    p_g(x) & : [0,1] \mapsto \mathbb{R}^+ \\
    p_g(x) & = 0.625 * \mathbbm{1}[0 \leq x \leq 0.4] + 1.875*\mathbbm{1}[0.6 \leq x \leq 1] \\
    & = \epsilon_\mathcal{D}*\mathcal{U}(0,0.4) + (1-\epsilon_{\mathcal{D}})*\mathcal{U}(0.6, 1)
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        p_{g,f}(x) & : [0,1] \mapsto \mathbb{R}^+ \\
        p_{g,f}(x) & = p_g(x) \rvert f=0 \\
        p_{g,f}(x) & = \mathcal{U}(0, 0.4)
    \end{split}
\end{equation}
\begin{equation}
    \begin{split}
        p_{g,s}(x) & : [0,1] \mapsto \mathbb{R}^+ \\
        p_{g,s}(x) & = p_g(x) \rvert f=1 \\
        p_{g,s}(x) & = \mathcal{U}(0.6, 1)
    \end{split}
\end{equation}
In words: $p_{g,f}$ is the conditional density of $g(Y)$ given that $Z$ is a failure; $p_{g,s}$ is the conditional density of $g(Y)$ given that $Z$ is a success. Note that this isn't a pathological case; in fact, it is possible to learn the correct decision rule exactly (i.e. ``if $g(Y) < 0.5$, output warning 1, otherwise output 0"). However, we assume that we do not know that this is the true distribution \textit{a priori}, and thus cannot use this as the warning system designer. \\

\noindent Now, assume the data for the training set of size $T$ is drawn iid from $\mathcal{D}$, and fix $\epsilon^*$. Consider the probability that Algorithm 1 fails to be $\epsilon^*$-safe. 
\begin{equation}
    \begin{split}
        & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \text{Algorithm is unsafe} \Big] \\
        = & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \underset{(Y',Z') \sim \mathcal{D}}{\mathbb{P}}\big[q > 1-\epsilon \rvert f=0\big] > \epsilon^* \Big] \\
        \geq & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \underset{(Y',Z') \sim \mathcal{D}}{\mathbb{P}}\big[q = 1 \rvert f=0\big] > \epsilon^* \Big]
    \end{split}
\end{equation}
Now, for a uniform conditional distribution $p_{g,f}$, the event 
\begin{equation*}
    \Big[ \underset{(Y',Z') \sim \mathcal{D}}{\mathbb{P}}\big[q = 1 \rvert f=0\big] > \epsilon^* \Big]
\end{equation*}
occurs when (per the paper notation of $\mathcal{A}$ being the failure set)
\begin{equation*}
    \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*}
\end{equation*}
where $Q_{1-\epsilon^*}$ is the $1-\epsilon^*$ quantile \sush{What is $Q_{1-\epsilon^*}$ a quantile of? As in which distribution (or sampling)?}. Thus, 
\begin{equation*}
    \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*} \implies \Big[ \underset{(Y',Z') \sim \mathcal{D}}{\mathbb{P}}\big[q = 1 \rvert f=0\big] > \epsilon^* \Big]
\end{equation*}
But because the conditional distribution is uniform, and the data is sampled i.i.d., we have that the former event occurs, for any fixed sample, w.p. $(1-\epsilon^*)^{\lvert \mathcal{A} \rvert}$ (of course, $\lvert \mathcal{A} \rvert$ is also a random variable over the samples). Summarizing the result so far and continuing the analysis, we have that
\begin{equation*}
    \begin{split}
        & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \text{Algorithm is unsafe} \Big] \\
        \geq & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \underset{(Y',Z') \sim \mathcal{D}}{\mathbb{P}}\big[q = 1 \rvert f=0\big] > \epsilon^* \Big] \\
        \geq & \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*} \Big] \\
        = & \sum_{t=0}^T \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*} \big\rvert \lvert \mathcal{A} \rvert = t \Big] \mathbb{P}[\lvert \mathcal{A} \rvert = t] \\
        = & \sum_{t=t_{min}}^T \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*} \big\rvert \lvert \mathcal{A} \rvert = t \Big] \mathbb{P}[\lvert \mathcal{A} \rvert = t] \\
        \geq & \mathbb{P}[\epsilon^* \text{ is valid}] \sum_{t=0}^T \underset{S \sim \mathcal{D}^T}{\mathbb{P}}\Big[ \max_{a \in \mathcal{A}} g(Y_a) < Q_{1-\epsilon^*} \big\rvert \lvert \mathcal{A} \rvert = t \Big] \mathbb{P}[\lvert \mathcal{A} \rvert = t] \\
        = & \mathbb{P}[\epsilon^* \text{ is valid}] \sum_{t=0}^T (1-\epsilon^*)^t {T \choose t} \epsilon_{\mathcal{D}}^t(1-\epsilon_\mathcal{D})^{T-t} \\
        \geq & \mathbb{P}[\epsilon^* \text{ is valid}] (1-\epsilon^*)^T \sum_{t=0}^T {T \choose t} \epsilon_{\mathcal{D}}^t(1-\epsilon_\mathcal{D})^{T-t} \\
        = & \mathbb{P}[\epsilon^* \text{ is valid}] (1-\epsilon^*)^T \\
        > & 0
    \end{split}
\end{equation*}

\noindent The progression to the fourth line follows from explicitly considering the set of $\lvert \mathcal{A} \rvert$ for which the $\epsilon^*$ is valid. This induces a $t_{min}$ in the sum (assume for invalid $t$, that the first term has probability 0), which is equivalently represented by an appropriate scaling of the entire sum introduced in the fifth line. \\

\noindent We choose the following parameters as an example: $T = 500$, $\epsilon_\mathcal{D} = 0.25$, $\epsilon^* = 0.015$. \\

\noindent Then, we have that the probability over $S \sim \mathcal{D}^T$ that $\epsilon^*$ is valid is greater than (1 - 1e-10) (calculated as 1 minus the probability that a value $X$ drawn from Bin$(T=500$, $\epsilon_\mathcal{D}=0.25)$ is less than 67), and that $(1-\epsilon^*)^T > 0.00051$. Therefore, we conclude that w.p. $> 0.0005$, over training sets of $T$ samples drawn i.i.d. from $\mathcal{D}$, the resulting algorithm will violate $\epsilon^*$ safety on a random, failing test sample drawn from $\mathcal{D}$. Of course, this probability is not tight at all. A back of the envelope calculation of the true probability of the algorithm failing is $\approx$ 0.15 (which is non-trivial?)





% 
% Ignore this section 
% 
\iffalse
\section{Concrete Example}
Consider the true distribution $p_g(g')$ comprised of the weighted union of the two conditionals, where $p_{g,f}(g') \sim \mathcal{U}(0, 0.4)$, $p_{g,s}(g') \sim \mathcal{U}(0.6, 1)$, and let $f=g$, $f_0 = 0.5$. We let the true expected failure rate over samples $(Y,Z) \sim \mathcal{D}$ be $\epsilon_\mathcal{D} = 0.25$. We note that $\epsilon_\mathcal{D}$ appears to be essentially independent of the actual guarantee and only affects the convergence by a constant. Thus, 
\begin{equation}
    p_g(g') = 0.25p_{g,f} + 0.75p_{g,s}
\end{equation}

Assume that we have a set $S$ of $T$ samples, of which there are $\lvert \mathcal{A} \rvert$ failures. Assume we want to show $\epsilon^*$ safety, and thus choose $\epsilon = \epsilon^* - \frac{1}{1 + \lvert \mathcal{A} \rvert}$. The fundamental question seems to be how they get $\mathcal{O}(1/T)$ concentration using conformal prediction (because $\lvert \mathcal{A} \rvert \rightarrow \epsilon_\mathcal{D}T = \mathcal{O}(T)$ as $T$ grows large).

\subsection{Case 1: The Result Holds For All Draws $\{(Y,Z)_t\}_{t=1}^T$, i.e. wp 1}

This seems impossible, for the reason mentioned above: if it holds for all draws, we can (I think?) try to construct a bad draw. Namely, w.p. $\geq (1-\epsilon^*)^{\lvert \mathcal{A}\rvert}$ over the sample $S$, every failing draw will lie below the $(1-\epsilon^*)$ quantile of $p_{g,f}$, and thus w.p. $\geq \epsilon^*$, the algorithm will output a false negative conditioned on a failing test sample $(Y',Z') \sim \mathcal{D}$. 

\subsection{The Result Holds in Expectation Over Draws} Therefore, it seems that the guarantee needs to be in expectation over both the algorithm randomness AND the sample $S \sim \mathcal{D}^T$. But then it seems we are missing a w.h.p. to concentrate the sample to the true distribution? (This is basically what PAC-Bayes needs to do, right?). But then it seems that even with the stronger i.i.d. assumption, the best one could do would be a Bernstein-like Inequality over the failure cases to concentrate $\hat{p}_{g,f}$ to the true conditional distribution $p_{g,f}$, which 
\begin{itemize}
    \item Holds w.h.p. (not w.p. 1)
    \item Still only attains $\mathcal{O}(1/\sqrt{T})$ convergence
\end{itemize}

\fi

==> deprecated/other.tex <==

\iffalse
\subsection{Decoupling the Detector's Loss}
In our setup, an error of $0$ is achieved if the failure detector is \emph{correct}, not just if a failure was going to occur and the detector predicted the event. Consider the following example: the failure detector always says there will be a failure. Then, deploying the conservative policy will prevent failures in all test environments; however, it will also always prevent robot from completing the task. Thus it would be interesting to study the improved effectiveness of the policy including the failure detector and conservative policy. % We will say the failure detector is perfect if the conservative policy is only deployed when a crash was going to occur. This ensures the maximum number of tasks are completed while completely avoiding failures. 

% Given the training data $S$, we can estimate the probability that the policy will fail running the standard policy $\pi$ while allowing for failures, but noting if the failure detector indicated the occurrence of a failure. 
Let $p$ be the probability that policy $\pi$ fails on $\D$, and $\widehat{p}$ be the probability that policy $\pi$ fails on $S$. A false positive (fp) corresponds to the detector indicating a failure when the policy did not fail. A false negative (fn) indicates a failure from the policy but no detection. A perfect detector will have a 0 fp and fn rate are 0. Let the probability of a fp and fn be $p_{\text{fp}}$ and $p_{\text{fn}}$ respectively. We then have probabilities for the 4 cases (assuming the conservative policy stops the task and -- no failure occurs but the task is not completed). Let FD be the failure detector.
\begin{enumerate}
    \item The FD is too conservative -- the policy would have succeeded but the FD guesses that a failure will occur: $p_{\text{fp}}$
    \item The FD is correct about no failure occurring: $1 - p - p_{\text{fp}}$ 
    \item The FD is correct that a crash will occur, and saves the policy from failing: $p - p_{\text{fn}} $
    \item The FD misses a policy failure: $p_{\text{fn}}$
\end{enumerate}
Here the error we wrote above is Case 1 + Case 4 or $p_{\text{fp}} + p_{\text{fn}}$, i.e., when the failure detector is incorrect about when a failure or success occurs. Are there ways to provide guarantees on any of the other quantities? $p_{\text{fn}}$ is of particular interest because it can represent the probability of failure when we use the failure detector in practice. However it's important to not allow the detector to become too conservative. Thus I think it makes sense to train with the case 1 + case 4 loss and then compute bounds for whichever thing we are interested. 

% Suppose we split our training dataset into two sets. $S_f$ is the set of environments on which the policy will fail, $S_s$ is the set of environments on which the policy will succeed. Note that $|S_f| = |S|*\widehat{p}$. \begin{equation}
%     \widehat{p}_{\text{fn}} \text{ (empirically on }S_f) =\frac{1}{n}\sum_{E \in S_f} C_{\pi}(f; E)
% \end{equation}
% and 
% \begin{equation}
%     \widehat{p}_{\text{fp}} \text{ (empirically on }S_s)=\frac{1}{n} \sum_{E \in S_s}C_{\pi}(f; E).
% \end{equation}
We can compute a PAC-Bayes bound on either of these quantities and bound the false-negative and false-positive rate directly. Let $C^{\text{fn}}_\pi(f;E)$ be the cost which assigns a $1$ only when Case 4 occurs (i.e. a false negative occurs). Thus $p_{\text{fn}} = \EE_{E\sim \D}C^{\text{fn}}_\pi(f;E)$. Then with high probability over a sampling of $S \sim \D$:
\begin{equation}
        p_{\text{fn}} = \underset{E \sim \D}{\EE}  C^{\text{fn}}_\pi(f; E) \leq  \underbrace{\frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E)}_{\widehat{p}_{\text{fn}}} + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{equation}

%\ds{Just wanted to add a comment about some possible additional quantities of interest. Specifically, I wonder if there might be some value in also considering the conditional probabilities. Something like $p_{n\rvert f}$ (the probability of a negative result given failure) might be relatable in some way to existing learning or statistical mechanisms. Such a quantity will almost certainly be dependent on the much smaller quantity $n_f$ (rather than the total number of samples); however, it seems to represent more fully the `gain' of the detector. Using the unconditioned $p_{nf}$ is of course fundamentally the same (just scaled down by the true expected fraction of failures over the distribution). I don't have a sense, though, of whether the bounds are sensitive to this.} \\

%\ds{Additionally, the practical use of the detector might be demonstrated effectively by an ROC-like curve of $p_{n \rvert f}$ vs $p_{p \rvert s}$. When there are no false negatives, we expect that the algorithm is just always guessing failure and thus the rate of false positives should be high. Similarly, with many false negatives, we would (hope) that at least the false positives should be low. But if the curve `bends in the right direction' it would suggest that more false negatives can be eliminated without sacrificing as much.}


We can try to get a bound on the probability of a false positive, conditioned on an environment causing a failure, since it may be scaled more appropriately than $p_{\text{fn}}$. Starting with the bound on $p_{\text{fn}}$ which holds with high probability over a sampling of $S \sim \D$
\begin{align}
        \underset{E \sim \D}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}} \\ \underbrace{p_s\underset{E \sim \D_s}{\EE}  C^{\text{fn}}_\pi(f; E)}_{=0} + p_f\underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}} \\
        p_f\underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) & \leq  \frac{1}{n} \sum_{E\in S_f} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{align}
However we do not know $p_f$ so we lower bound it by $\bar{p}_f$ with probability $1-\delta'$. With a union bound we can say the following with probability at least $1 - \delta' - \delta$ over a sampling of $S \sim \D^n$:
\begin{equation}
    \underset{E \sim \D_f}{\EE}  C^{\text{fn}}_\pi(f; E) \leq  \frac{1}{\bar{p}_f n} \sum_{E\in S_f} \underset{f \sim F}{\EE} C^{\text{fn}}_\pi(f;E) + \frac{1}{\bar{p}_f}\sqrt{\frac{\KL(F \| F_0) + \ln\frac{2\sqrt{n}}{\delta}}{2n}}
\end{equation}
Now let's bound $p_f$ with a standard concentration inequality: \alec{I think this is right but will check}
\begin{align}
    P\big[p_f \geq \widehat{p}_f - t \big] \geq 1 - e^{-2nt^2}  \\
    P\Bigg[p_f \geq \underbrace{\widehat{p}_f - \sqrt{\frac{\ln(\frac{1}{\delta'})}{2n}}}_{\bar{p}_f} \Bigg] \geq 1 - \delta'
\end{align}
However, if $\widehat{p}_f - \sqrt{\frac{\ln(\frac{1}{\delta'})}{2n}} \leq 0$, then our guarantee is vacuous! Thus, this will not work for very small $p_f$. 
\alec{@David, I think you're right that we probably can't do any better than this. It would be weird if we could avoid a second $\delta$ and a union bound all together. If things were conditioned on the distribution over the failure detector (instead of the distribution over samples) we could use the a data-processing inequality and not need a union bound (which is more like what I did in the PAC-BUS paper)... as it stands I still think this is cool, perhaps useful even though we compute it by directly loosening the bound on the false-negative rate.}

\fi
